Evidence for a Z < 8 Origin of the Source Subtracted Near Infrared Background

This letter extends our previous fluctuation analysis of the near infrared background at 1.6 microns to the 1.1 micron (F110W) image of the Hubble Ultra Deep field. When all detectable sources are removed the ratio of fluctuation power in the two images is consistent with the ratio expected for faint, z<8, sources, and is inconsistent with the expected ratio for galaxies with z>8. We also use numerically redshifted model galaxy spectral energy distributions for 50 and 10 million year old galaxies to predict the expected fluctuation power at 3.6 microns and 4.5 microns to compare with recent Spitzer observations. The predicted fluctuation power for galaxies at z = 0-12 matches the observed Spitzer fluctuation power while the predicted power for z>13 galaxies is much higher than the observed values. As was found in the 1.6 micron (F160W) analysis the fluctuation power in the source subtracted F110W image is two orders of magnitude below the power in the image with all sources present. This leads to the conclusion that the 0.8--1.8 micron near infrared background is due to resolved galaxies in the redshift range z<8, with the majority of power in the redshift range of 0.5--1.5.

==> README <==
*********************Referee's Report*************************************

The paper 'Evidence for Low Redshift Origin of the Source Subtracted Near 
Infrared Background' by Thomson et al. shows that the fluctuation power in
the HUDF at 1.1 and 1.6 \mum after subtraction of all detectable sources is 
inconsistent with a large contribution from galaxies at z>8.  This conclusion is 
obtained by comparing the color of residual fluctuation in the 1.1 and 1.6 
\mum HUDF images with numerically redshifted galaxy SED.  Moreover this 
conclusion is supported by the comparison with recent background fluctuation
detection at 3.6 and 4.5 \mum obtained with Spitzer.

The paper is timely and original.  It warrants publication in ApJ but I do
not see the urgency for a publication as a Letter (see also my GENERAL
COMMENT a).



1. GENERAL COMMENT
a) I find the paper a quite difficult read:  the main difficulty arises 
from the fact that many important pieces of information are not explicitely 
given in the paper.  The reader is often referred to previous papers of the 
same authors in order to relevant details about data analysis, source 
subtraction, source redshift distribution, background intensity, SED 
calculation,... Moreover, the introduction section is too short and generic 
(see SPECIFIC MAJOR POINT a) . 
I guess that this problem is partly due to the tight constraints set by the 
ApJ Letter format.  I suggest that the authors consider the idea of expanding 
the paper and re-submitting it for publication in the ApJ Part 1.

REPLY: The referee is correct that we condensed several areas to fit within
the Letter constraints.  In responding to the referee's suggestions we have
relaxed that constraint and the current length is probably beyond the letter
allocation.  We presume that the editor will send it to the main journal if
that is the case.  

b) I am confused by authors use of the expression 'low redshift galaxies'. 
The final conclusion of the paper is that fluctuations from unresolved
sources can be due to faint galaxies in the redshift range z=1-8. For a large
part of the astrophysical community, galaxies at z>3 are high-redshift objects!
I suggest to change the expression 'faint, low redshift galaxies' with 
'faint galaxies in the redshift range 1<z<8'. Also, I suggest to change the
title accordingly.

REPLY: We have changed the references to "low redshift galaxies" to "z<8".
Our original term was in response to suggestions that the galaxies responsible
for the source subtracted fluctuations were at redshifts above 10.

2. SPECIFIC MAJOR COMMENTS
a) The introduction should include sufficient introductory material and 
background explanation for readers who are not specialists in the field.
Some more details should be given about the existence (or not) of a NIRB 
intensity excess and about the detections of residual fluctuations at 
different wavelengths.

REPLY: We have added details of the analysis in our first paper in the
introduction.
 
Moreover, a brief summary of the discussion on the interpretation of the
residual fluctuation origin appears necessary.  Stating that "the 
interpretation (of Kashlinsky et al. 2007a) has been challenged by Cooray et 
al, with  a reply to the challenge by Kashlinsky et al. (2007)" does not
help the reader to understand what are the main points of the discussion.

REPLY: We have added a discussion of the interpretation of the fluctuations
to the introduction.


Finally, reference to other works that have provided different interpretations 
should be given.  For example, Salvaterra+ (2006, MNRAS, 368, L6) have shown that 
the unresolved fluctuations observed by Spitzer could be accounted for by 
normal (i.e. hosting PopII stars) galaxies at z>=5.  B.t.w., this conclusion 
is not at odds with (in fact, it supports) the main conclusions of the present 
paper.

REPLY: We have added a reference to the Salvaterra 2006 work in the introduction.
Thanks to the referee for calling it to our intention.  The paper came out during
the extensive discussions with the referee on the first paper.  We had intended
to include it in this paper but it got missed.

b) Expand Sect. 2.1.  Since a crucial confirmation of the conclusions 
comes from the comparison of HUDF and Spitzer residual fluctuation,
some more details on the compatibility of different data sets are needed. 
In particular, the use of ACS images to remove sources from NICMOS images 
should be illustrated more extensively.  Are the subtraction levels really 
comparable?  How does the result depend on the adopted SED? Could the excess of
fluctuations in the 3.6 \mum predicted for template 6 be caused by
a different subtraction limit?

REPLY: We have greatly expanded the discussion on the subtraction levels
in section 3.1 which has been moved from its original position to after
the discussion of the fluctuation colors.  We have added a figure (Figure 4)
to show the subtraction levels as a function of redshift for the F775W band,
the band we had shown the detection levels for in the Thompson et al. 2006
NUDF paper.  The answer is that the subtraction levels are equal except for
the very highest redshift galaxies that have no flux in the ACS bands. 

c) Give more details on the adopted SED templates: e.g. specify the adopted 
IMF and metallicity values.  How do authors model IGM absorption? 

REPLY: We have added more details on the adopted SED templates in section 3.
We also added figure 2 to show the template distribution and Table 1 that gives
the SED properties.  We have also added a reference to Madau et al. 1996
which is the source of our calculation of the IGM absorption.

d) The color results are quite insensitive to the actual redshift of the main 
sources of fluctuations, as long as their redshift is <8.  Can the authors  
speculate on what theoretical and/or observational features may be useful  
to disentagle low-redshift (i.e. z<5) and high redshift (z>5) contributions?

REPLY: It may be possible to do a fluctuation analysis on the ACS images
as well to get color information to do a fluctuation photometric redshift.  
Since we used the HUDF team prepared ACS images we did not have
the very detailed knowledge of how they were produced and felt that analysis
was beyond the scope of this paper.

d) In Fig. 3 an upper limit of the fluctuation power from 1.1 mum dropout is 
given.  As stated in Sect. 3.1, this limit is still above the Gaussian noise 
spectrum.  Quantify the fluctuation excess that is possibly due to very high 
redshift galaxies on the basis of this finding.

REPLY: We have added that discussion as the fourth paragraph in section 3.2.


3. MINOR COMMENTS
a) The quality of Fig. 2 is very low.  Please cut the y-axis to a value of ~10.
in order to improve the presentation of the results.

REPLY: We have cut the axis to a value of 10.

b) Sect. 3: '.. the predominant SED for faint galaxies at Z>0.5'. Is Z 
metallicity or redshift?

REPLY: It is redshift and we now indicate so in the text.

c) Please, check carefully the text. I find many typos. Here I list just a few 
examples:
     - Sect. 3: \mu instead of \mu m 
     - Sect. 3.1 :'...we cannot make a the same argument...'
     - References: angstrom instead of A&A

REPLY: We have corrected these and other typos.  Thanks to the referee for the 
very helpful comments.

